Fast Converging Anytime Model Counting

Model counting is a fundamental problem which has been influential in many applications, from artificial intelligence to formal verification. Due to the intrinsic hardness of model counting, approximate techniques have been developed to solve real-world instances of model counting. This paper designs a new anytime approach called PartialKC for approximate model counting. The idea is a form of partial knowledge compilation to provide an unbiased estimate of the model count which can converge to the exact count. Our empirical analysis demonstrates that PartialKC achieves significant scalability and accuracy over prior state-of-the-art approximate counters, including satss and STS. Interestingly, the empirical results show that PartialKC reaches convergence for many instances and therefore provides exact model counting performance comparable to state-of-the-art exact counters.

==> sections/Experiments.tex <==
\begin{table*}[tb]
	\centering
	%\footnotesize
	\aboverulesep = 0.2ex
	\belowrulesep = 0.2ex
	%\captionsetup{width = 95mm}
	%\belowcaptionskip = 125mm
	%\renewcommand{\arraystretch}{1.5}
	\begin{tabularx}{\linewidth}{l>{\centering\arraybackslash}*{10}{>{\centering\arraybackslash}X}}\toprule
		\multirow{3}*{domain (\#, \#known)} & \multicolumn{3}{c}{exact} & \multicolumn{7}{c}{approximate} \\\cmidrule(rl){2-4}\cmidrule(rl){5-11}
		{} & \multirow{2}*{D4} & \multirow{2}*{\hspace{-0.65cm} sharpSAT-td} & \multirow{2}*{ExactMC} & \multicolumn{3}{c}{\PartialKC{}} & \multicolumn{2}{c}{satss} & \multicolumn{2}{c}{STS} \\\cmidrule(rl){5-7}\cmidrule(rl){8-9}\cmidrule(rl){10-11}
		{} & {} & {} & {} & \#approx & \#conv & $\varepsilon=5$ & \#approx & {$\varepsilon=5$} & \#approx & {$\varepsilon=5$} \\\midrule
		%domain (\#) & \LOBDDC{}{}/LLY & \LSDD{}/miniC2D & \RoneK{1}/Panini & \dDNNF{}/dsharp &  \dDNNF{}/d4 \\\midrule
		Bayesian-Networks (201, 186)  & 179 & \textbf{186} & \textbf{186} & \textbf{195} & \textbf{186} & \textbf{186} & 18 & 17 & 157 & 148 \\
		BlastedSMT (200, 183) & 162 & 163 & 169 & \textbf{200} & 167 & 177 & 150 & 129 & \textbf{200} & \textbf{178} \\
		Circuit (56, 51) & 50 & 50 & \textbf{51} & \textbf{54} & 50 & 50 & 15 & 13 & 50 & 44 \\
		Configuration (35, 35) & \textbf{34} & 32 & 31 & \textbf{35} & 29 & 33 & 33 & 31 & 35 & 12 \\
		Inductive-Inference (41, 23) & 18 & 20 & 22 & 37 & 20 & \textbf{23} & 40 & 19 & \textbf{41} & \textbf{23} \\
		Model-Checking (78, 78) & 75 & 77 & \textbf{78} & \textbf{78} & 77 & \textbf{78} & 11 & 7 & 9 & 7 \\
		Planning (243, 219) & 208 & \textbf{214} & 213 & \textbf{239} & 209 & 213 & 169 & 126 & 238 & 103 \\
		Program-Synthesis (220, 119) & 91 & 77 & 107 & \textbf{135} & 99 & \textbf{111} & 81 & 64 & 120 & 106 \\
		QIF (40, 33) & 29 & 28 & 32 & \textbf{40} & 23 & \textbf{32} & 15 & 13 & 27 & 25 \\
		MC2022\_public (100, 85) & 72 & 76 & 76 & \textbf{87} & 69 & \textbf{78} & 53 & 45 & \textbf{87} & 77 \\\midrule[0.02em]
		Total (1214, 1012) & 918 & 923 & 965 & \textbf{1100} & 929 & \textbf{981} & 585 & 463 & 957 & 722 \\\bottomrule
	\end{tabularx}
	\caption{Comparative counting performance between Ganak, c2d, D4, ExactMC, satss, STS, and \PartialKC{}, where each cell below tool refers to the number of solved instances}
	%	under the given conditions} 
	\label{tab:expri:counting}
\end{table*}

\section{Experiments}
\label{sec:experiments}

\ry{what parameters in PartialKC - isn't the N needed? Shouldnt there
be a ApproxMC comparison with epsilon and delta to match?}
We evaluated {\PartialKC}
on a comprehensive set consisting of two parts: 1114 benchmarks from a wide range of application areas, including automated planning, Bayesian networks, configuration, combinatorial circuits, inductive inference, model checking, program synthesis, and quantitative information flow (QIF) analysis; and 100 public instances adopted in Model Counting Competition 2022. We remark that the previous 1114 instances have been employed in the past to evaluate model counting and knowledge compilation techniques~\cite{D4,Lai:etal:17,Fremont:etal:17,ApproxMC3,Lai:etal:21}. 
% In this section, we first evaluate the performance of compiling time and compilation sizes of \panini{}; and then apply \panini{} to then 
% a reasoning task applicable to probabistic methods, 
% e.g. probabilistic databases, probabilistic programming and tractable learning.
% \todo{some benchmarks are not available}
The experiments were run on a cluster\footnote{
The cluster is a typical HPC cluster where jobs are run through a job queue.
}
where each node has 2xE5-2690v3 CPUs with 24 cores and 96GB of RAM. 
Each instance was run on a single core with a timeout of 3600 seconds and 8GB memory.

We compared exact counters D4 \cite{D4}, sharpSAT-td \cite{SharpSAT-TD}, and ExactMC \cite{Lai:etal:21}, and approximate counters satss \cite{Gogate:Dechter:11} and STS \cite{STS}.
We remark that both satss and STS are anytime.
We used the widely employed pre-processing tool B+E \cite{BplusE} for all the instances, which was shown very powerful in model counting.

Table \ref{tab:expri:counting} shows the performance of the six counters.
The results show that \PartialKC{} can solve approximately much more instances than the other five tools.
We emphasize that there are 116 instances that was solved by none of D4, sharpSAT-td, and ExactMC.
Since \PartialKC{} gives an unbiased estimate about the exact count, we can immediately obtain probabilistic lower bounds of counts by utilizing Markov's inequality for those instances.
The results also show that \PartialKC{} can get convergence on 929 instances; that is, we can get the exact counts for these instance, and therefore outperformed D4 and sharpSAT-td.
In order to evaluate the accuracy of \PartialKC{}, we employed D4, sharpSAT-td, and ExactMC, respectively, to solve each instance with a bigger timeout 14400 seconds.
Therefore, we exactly solved 26 more instances, and the numbers of solved instances are marked in the first column in Table \ref{tab:expri:counting}.

We compare the convergence performance of \PartialKC{}, satss, and STS further on three selected instances depicted in Figure \ref{fig:convergence}.
Figure \ref{fig:convergence} PartialKC gets fast convergence, while neither satss nor STS gets convergence.

\begin{figure*}[htbp]
	\centering
	\subfloat[inductive-inference\_ii32e1]{\label{fig:convergence:a}
		\centering
		\begin{minipage}[c]{0.33\linewidth}
			\centering
			\includegraphics[width = \textwidth]{inductive-inference_ii32e1.pdf}
		\end{minipage}
	}
	\subfloat[Planning\_prob005.pddl]{\label{fig:convergence:b}
		\centering
		\begin{minipage}[c]{0.33\linewidth}
			\centering
			\includegraphics[width = \textwidth]{Planning_prob005.pddl.pdf}
		\end{minipage}
	}
	\subfloat[ProgramSynthesis\_sygus\_15A-4]{\label{fig:convergence:c}
		\centering
		\begin{minipage}[c]{0.33\linewidth}
			\centering
			\includegraphics[width = \textwidth]{ProgramSynthesis_sygus_15A-4.pdf}
		\end{minipage}
	}
	\caption{The convergence performance of \PartialKC{}, SampleSearch and SearchTreeSampler over three instances with known counts depicted by straight horizontal lines. (Best viewed in color)}\label{fig:convergence}
\end{figure*}

\begin{figure}[htbp]
	\centering
	\includegraphics[width = \linewidth]{accelaration.pdf}
	\caption{The accelaration performance of the calling of \MicroKC{}. (Best viewed in color)}\label{fig:accelaration}
\end{figure}

